Lagrangian cobordisms, Lefschetz fibrations and quantum invariants

We study Lagrangian cobordisms with the tools provided by Lagrangian quantum homology. In particular, we develop the theory for the setting of Lagrangian cobordisms or Lagrangians with cylindrical ends in a Lefschetz fibration, and put the different versions of the quantum homology groups into relation by a long exact sequence. We prove various practical relations of maps in this long exact sequence and we extract invariants that generalize the notion of discriminants to Lagrangian cobordisms in Lefschetz fibrations. We prove results on the relation of the discriminants of the ends of a cobordism and the cobordism itself. We also give examples arising from Lagrangian spheres and relate the discriminant to open Gromov Witten invariants. We show that for some configurations of Lagrangian spheres the discriminant always vanishes. We study a set of examples that arise from Lefschetz pencils of complex quadric hypersurfaces of the complex projective space. These quadrics are symplectic manifolds endowed with real structures and their real part are the Lagrangians of interest. Using the results established in this thesis, we compute the discriminants of all these Lagrangians by reducing the calculation to the previously established case of a real Lagrangian sphere in the quadric.

==> lefschetz.tex <==
% !TEX root = ../main.tex

\section{Lefschetz Fibrations}

In this section we adopt the constructions to the setting of a cobordism in a Lefschetz 
fibration. Throughout this section we borrow definitions, constructions and ideas 
from~\cite{BCLefschetz} respectively~\cite{BCLefschetzArxiv}.

Let us start with the definition of a Lefschetz fibration.
\begin{definition}\label{def:Lefschetz}
$\pi:E\to S$, where $E,\Omega_E$ the total space of the Lefschetz fibration.
 see~\cite{BCLefschetz} Def 2.1.1.
\end{definition}

The symplectic structure $\Omega_E$ defines a connection $\Gamma$ on $E\setminus 
Crit(\pi)$. 
It is defined by fixing its horizontal distribution. 
Let $T^v_x(E)$ be the vertical tangent space at $x\in E$, i.e. $T^v_x(E);=ker(d\pi_x)$.
Then define for every $x\in E\setminus Crit(\pi)$ the horizontal distribution at $p$:
$$\mathcal{H}_x:=\{u\in T_x(E)|\Omega_E(\xi,u)=0 \forall \xi\in T^v_x(E)\}.$$
In particular, for every $p\in E$ we have $T_pE\cong T_p^vE\oplus \mathcal{H}_x$ and 
$\mathcal{H}_x\cong T_{\pi(p)}S$.
The connection $\Gamma$ induces a parallel transport. 
For a smooth path $\lambda:[a,b]\to \mathbb{C}\setminus Critv(\pi)$ let 
$\Pi_{\lambda}:E_{\lambda(a)}\to E_{\lambda(b)}$ be the parallel transport along 
$\lambda$.

\begin{assumption}\label{assum:Lefschetz}
 For now we assume that 
\begin{enumerate}
 \item The Riemann surface $(S,j)$ is the standard complex plane $(\mathbb{C},i)$.
 \item There exists exactly one critical point $q\in Crit(\pi)$ and we may assume that 
$pi(q)=0$.
\end{enumerate}
\end{assumption}

\begin{lemma}
 Under the above assumptions~\ref{assum:Lefschetz}, there exists a deformation retraction 
$r:E\to F_0$. 
\end{lemma}

\begin{proof}
 Consider the vector field on $\mathbb{C}$ given by
$$w(z):=-\nabla r^2,$$
where $z=re^{i\phi}$.
We can lift the vector field horizontally with the distribution defined above to obtain a 
vector field $v$ on $E\setminus q$. 
Notice that the flow $\phi_v^t$ of $v$ preserves the fibers, i.e. 
$$\phi_v^t(F_b)=(F_{b'})\text{ and } \sigma_b=(\phi^t_v)^*(\sigma_{b'})$$
where $\sigma_b$ and $\sigma_{b'}$ are the symplectic structures on the fibers $F_b$ and 
$F_{b'}$ respectively induced by $\Omega_E$.

We would like to extend the vector field $v$ to all of $E$.
For this consider a curve $\gamma:[0,1]\to E$ such that $\gamma(0)\in F_0$ lies in the 
singular fiber over $0$.
Notice that $\pi\circ\gamma(t))$ is a smooth curve in $\mathbb{C}$ such that 
$\pi\circ\gamma(0)=0$ and the vector field $w$ vanishes at $0$ with all its 
derivatives.
Hence we compute
\begin{equation}
 \begin{array}{ccc}
  \frac{\partial ^n}{\partial t^n}|_{t=0}(v(\gamma(t))&=&\frac{\partial ^n}{\partial 
t^n}|_{t=0}(w(\pi\circ \gamma(t)),0)\\
&=& (0,0).\\
 \end{array}
\end{equation}
Thus we can extend $v$ smoothly to all of $E$ by setting $v(p)=0$ for all $p\in F_0$.
then 
$$\lim_{t\to \infty} \phi^t_v(E)=F_0$$
$$\phi^t_v|_{F_0}=Id_{F_0}$$
and $$\phi^0_v=Id_E.$$
This proves the Lemma.
\end{proof}

Let $0\neq p\in \mathbb{C}$ 
and let $C\in F_p$ denote the vanishing cycle. It is well-known that the vanishing cycle 
is a Lagrangian sphere and in particular has self-intersection equal to minus its Euler 
characteristic. I.e. $L\cdot L=-\chi(L)=-(1+(-1)^n))$.

\begin{lemma}
 Under the assumptions~\ref{assum:Lefschetz}, the reduced singular homology of the total 
space $E$ is
$$\tilde{H}_*(E)\cong \tilde{H}_*(F_p,C).$$
\end{lemma}

\begin{proof}
 We know from Picard Lefschetz Theory that $F_0\cong F_p/C$. 
By the previous Lemma and general methods from Algebraic Topology we see that
$$\tilde{H}_*(E)\cong \tilde{H}_*(F_0)\cong \tilde{H}_*(F_p/C)\cong \tilde{H}_*(F_p,C).$$
\end{proof}

\subsection{The Ambient Quantum Homology of a Lefschetz fibration with one critical point}

We start with the local model. 
Consider the Lefschetz fibration
\begin{equation}
 \begin{array}{ccc}
  \pi:\mathbb{C}^n &\to& \mathbb{C}\\
      (z_1,\ldots,z_{n+1}) &\mapsto& z_1^2+\ldots z_{n+1}^2.\\
 \end{array}
\end{equation}
It has a single isolated critical point at $0$.
Let $\gamma:[0,1]\to \mathbb{C}$ be the curve $t\mapsto e^{it2\pi}$.
Define $X:=\pi^{-1}(\gamma)$ and $F:=\pi^{-1}(e^{i2\pi})$.
The map 
$$\phi:=\pi_X:X\to S^1$$
is a fiber bundle.
Denote by $h_*:H_*(F)\to H_*(F)$ the monodromy given by the action of a generator of 
$\pi_1(S^1)$ on the homology of the fibers. Then $h^*$ is the characteristic 
homeomorphism of the fiber $F$.
More details about this fiber bundle and the monodromy can be found 
in~\cite{Milnor:singularpoints} and~\cite{Ebeling}.
In~\cite{Milnor:singularpoints} we also find the following useful Lemma.
\begin{lemma}[The Wang sequence]
To a fiber bundle $\phi:X\to S^1$ with fiber $F:=\phi^{-1}(1)$ and characteristic map 
$h_*$ 
there exists an associated exact sequence of the form
$$
\begin{tikzcd}
   \cdots \ar[r] & H_{*+1}(X) \ar[r] & H_*(F) \ar[r,"h_*-Id_{*}"] & H_*(F) \ar[r] & 
H_*(X)\ar[r] &\cdots 
  \end{tikzcd}
$$
\end{lemma}

\begin{proof}
Let $F_t$ be the fiber over the point $e^{i t 2\pi}$.
The covering homotopy $h_t:F\to F_t$, where $h_0=Id_F$ and $h_1=h$ induces a mapping 
$$F\times[0,1]\to X,$$
which induces and isomorphism 
$$H_*(F\times[0,1],F\times\{0\}\cup F\times\{1\})\to H_*(X,F).$$
But $H_{*-1}(F)\cong H_*(F\times[0,1],F\times\{0\}\cup F\times\{1\})$ and thus the long 
exact sequence of the pair $(X,F)$ gives the desired sequence.
\end{proof}

The following facts are well-known from in Picard Lefschetz theory and can be found in 
many sources, including~\cite{Ebeling} 
The fiber $F$ is diffeomorphic to the disc bundle $DS^n$ and hence $F$ has the homotopy 
type of a sphere $S^n$.
The homology $H_n(F)$ is generated by the homology class of the vanishing cycle $\Delta$.
The monodromy is the identity on $\Delta$.
Now consider the relative homology 
$$H_*(F,\partial F)\cong H_*(DS^n,\partial DS^n)\cong \begin{cases} \mathbb{Z} & *=n+1\\
                                                       0 \text{ otherwise}.
                                                      \end{cases}$$
Let $\Delta_*$ be a generator of $H_{n+1}(F,\partial F)$ such that $<\Delta_*,\Delta>=1$.
The monodromy $H_*$ acts on $H_*(F,\partial F)$ by $\Delta_*\mapsto \Delta_*$. 
Using these results form Picard Lefschetz theory we compute:
\begin{corollary}
 The relative homology of the space $X,\partial X$ is
$$H_*(X,\partial X)\cong \begin{cases}
                          \mathbb{Z} & *=n+1\\
0 & \text{ otherwise}
                         \end{cases}.$$
\end{corollary}
\begin{proof}
 Apply the Wang sequence to the fiber bundle $f:X/\partial X\to S^1$ with fiber $F$. 
\end{proof}

\begin{lemma}
 Consider the function
\begin{equation}
 \begin{array}{ccc}
  f:\mathbb{C}^n &\to& \mathbb{C}\\
      (z_1,\ldots,z_{n+1}) &\mapsto& |z_1|^2+\ldots |z_{n+1}|^2.\\
 \end{array}
\end{equation}
The Morse complex of this function computes $H_*(X,\partial X)$.
\end{lemma}

\begin{proof}
 Notice that $f(z_1,\ldots,z_{n+1})=z_1\overline{z}_1+\ldots+z_{n+1}\overline{z}_{n+1}$ 
and $$\nabla f=\left(
\begin{matrix}
    \overline{z}_1 \\
    z_1 \\
    \vdots \\
    \overline{z}_{n+1}\\
    z_n\\
\end{matrix}\right).$$
The Hessian matrix is 
$$Hf=\left(\begin{matrix} 0 & 1 & 0 & 0 & \ldots\\
            1 & 0 & 0 & 0 & \ldots \\
	    0 & 0 & \ddots & \ldots \\
	    \vdots & & & & \\
	    0 & 0 & \ldots & 0 & 1 \\
	    0 & 0 & \ldots & 1 & 0 \\
           \end{matrix}
\right),$$
which has the eigenvalues $1$ and $-1$ both of multiplicity $n+1$. Hence $f$ has a single 
critical point of index $n-1$.
\end{proof}

Let $\pi:E\to \mathbb{C}$ be a Lefschetz fibration.
Assume that assumption~\ref{assum:Lefschetz} holds. 
Locally around the critical point the Lefschetz fibration is a complex Morse function.
I.e. there exists an open neighborhood $U\cong \mathbb{C}^{n+1}$ of the critical point 
$p$ and an open set $V=\tilde{\pi}(U)\subset \mathbb{C}$ diffeomorphic to 
$\mathbb{C}$, such that $\pi|_U$ has the form
$$\tilde{\pi}:\mathbb{C}^{n+1}\to \mathbb{C}:(z_1,\ldots,z_{n+1})\mapsto 
z_1^2+\ldots+z_{n+1}^2.$$ 
Let $\gamma:S^1\to \mathbb{C}$ be a curve in the complex plane that has winding number 
one around zero. 
We may assume that $\gamma\subset V$. 
Define $X:=\pi^{-1}(\gamma)$ and consider the fiber bundle 
$$f:X\to S^1,$$
with fiber $F:=\pi^{-1}(\gamma(1))=f^{-1}(\gamma(1))$.
Denote by $h_*:H_*(F)\to H_*(F)$ the monodromy given by the action of a generator of 
$\pi_1(S^1)$ on the homology of the fibers. Then $h^*$ is the characteristic 
homeomorphism of the fiber $F$.
More details about this fiber bundle and the monodromy can be found 
in~\cite{Milnor:singularpoints} and~\cite{Ebeling}.
In~\cite{Milnor:singularpoints} we also find the following Lemma.
\begin{lemma}[The Wang sequence]
 To a fiber bundle $f:X\to S^1$ with fiber $F:=f^{-1}(1)$ and characteristic map $h_*$ 
there exists an associated exact sequence of the form
$$
\begin{tikzcd}
   \cdots \ar[r] & H_{*+1}(X) \ar[r] & H_*(F) \ar[r,"H_*-Id_{*}"] & H_*(F) \ar[r] & 
H_*(X)\ar[r] &\cdots 
  \end{tikzcd}
$$
\end{lemma}

\begin{proof}
Let $F_t$ be the fiber over the point $e^{i t 2\pi}$.
The covering homotopy $h_t:F\to F_t$, where $h_0=Id_F$ and $h_1=h$ induces a mapping 
$$F\times[0,1]\to X,$$
which induces and isomorphism 
$$H_*(F\times[0,1],F\times\{0\}\cup F\times\{1\})\to H_*(X,F).$$
But $H_{*-1}(F)\cong H_*(F\times[0,1],F\times\{0\}\cup F\times\{1\})$ and thus the long 
exact sequence of the pair $(X,F)$ gives the desired sequence.
\end{proof}

Let $\Delta\in H_n(F)$ denote the class of the vanishing sphere of the Lefschetz 
fibration $\pi:E\to \mathbb{C}$.
By Picard Lefschetz theory it is known that the fiber $\tilde{\pi}^{-1}(\gamma(1))$ is 
diffeomorphic to the disc bundle $DS^n$.
It is also well-known that the monodromy is isotopic to a diffeomorphism with compact 
support in $U$. 
In this local model we have
$$H_*(DS^n)\cong \begin{cases} \mathbb{Z} & *=0,n\\
                    0 & \text{ otherwise }
                   \end{cases}$$
and 
$$H_*(DS^n,\partial DS^n)\cong \begin{cases}
                                \mathbb{Z} & *=n\\
				0 &\text{ otherwise }
                               \end{cases}.$$
Let $\Delta^*$ denote the unique class in $H_*(DS^n,\partial DS^n)$, such that 
$<\Delta^*,\Delta>=1$. Notice that $H_*(DS^n,\partial DS^n)\cong \Delta^*\mathbb{Z}$. 
The monodromy $h_*$ acts on $H_*(DS^n,\partial DS^n)$ by $\Delta^*\mapsto \Delta^*$. 
\subsection{An Example}
\begin{example}
We investigate the example of real quadric surfaces, which was already studied 
in~\cite{BCLefschetzArxiv}. It is a real Lefschetz fibration associated to a pencil of 
complex quadric surfaces in $\mathbb{C}P^3$. 
For a detailed discussion of the construction the reader is referred 
to~\cite{BCLefschetzArxiv}.
The regular fibers of this Lefschetz fibration are symplectomorphic to 
$(\mathbb{C}P^1\times \mathbb{C}P^1,2\omega_{\mathbb{C}P^1}\oplus 
2\omega_{\mathbb{C}P^1})$.
One section defining a regular fiber is given by
$$\lambda_0(\overline{X})=X_0^2+X_1^2+X_2^2-X_3^2=0$$ 
Consider the singular fiber given by
$$X_0^2+X_1^2+X_2^2=0.$$ 
The vanish cycle in $\lambda_0$ is the Lagrangian sphere 
$$C=\{[X_1:X_2:X_3:1]\in \mathbb{C}P^3| X_0^2+X_1^2+X_2^2=1\}\cap \mathbb{R}P^3\subset 
\lambda_0.$$
The singular fiber $F_0$ in this example is given by 
$$X_0^2+X_1^2+X_2^2-X_3^2-2X_0X_3+2X_1X_2$$
which becomes 
$$\tilde{X_0}^2+\tilde{X_1}^2-\tilde{X}_3^2-2\tilde{X_0}\tilde{X_3}$$ 
after a suitable coordinate change.
In this coordinate system it is easy to see that this singular fiber is the cone over the 
conic $C:=\{\tilde{X}_0^2+\tilde{X}_1^2-\tilde{X}_3^2-2\tilde{X}_0\tilde{X}_3\}$ in 
$\mathbb{C}P^2\cong\{\tilde{X_2}=0\}$. 
The apex of this cone corresponds to the point that is obtained by collapsing the 
vanishing cycle in the singular fiber. 
Now $C$ is curve of degree two in $\mathbb{C}P^2$. 
Thus the normal bundle of $C$ is 
$$\mathcal{N}_C\cong\mathcal{N}_{\mathbb{C}P^2/\mathbb{C}P^3}|_{C}\cong 
\mathcal{O}(1)_{\mathbb{C}P^2}|_C\cong\mathcal{O}(2),$$
where the equality follows from the fact that $C$ has degree two.
Consider the two sections $\Sigma_2:=\mathbb{P}(0\oplus \mathcal{O})$ and 
$\Sigma_{-2}=\mathbb{P}(\mathcal{O}(2)\oplus 0)$. 
The homological self-intersections are $[\Sigma_2]\cdot [\Sigma_2]=2$ and 
$[\Sigma_{-2}]\cdot[\Sigma_{-2}]=-2$.
The singular fiber $F_0$ is thus almost a ruled surface. More precisely, it is 
obtained from $\mathbb{P}(\mathcal{O}(2)\oplus 
\mathcal{O})$ by collapsing the sphere $\Sigma_{-2}$. This sphere corresponds to the 
vanishing cycle in a regular fiber.
One can show that $F_0\cong\mathbb{P}(\mathcal{O}(2)\oplus \mathcal{O})/\Sigma_{-2}$ 
carries a canonical complex structure. \begin{bf}Where???\end{bf}

We can compute the Gromov-Witten invariants of $\mathbb{P}(\mathcal{O}(2)\oplus 
\mathcal{O})$ and then deduce from it the Gromov-Witten invariants of $F_0$.
It is known that the two sections $\Sigma_2$ and $\Sigma_{-2}$ have the relation
$$[\Sigma_2]=[\Sigma_{-2}]+2[F],$$
where $F$ is a fiber of the bundle $\mathbb{P}(\mathcal{O}(2)\oplus 
\mathcal{O})$.
A basis of $H_*(\mathbb{P}(\mathcal{O}(2)\oplus 
\mathcal{O}))$ is $\{p,F,\Sigma_2,U\}$, where $p$ is the class of a point and $U$ is 
the fundamental class.
\begin{remark}
 Usually the Gromov-Witten invariants are defined in terms of the cohomology. 
Given three homology classes $a,b,c\in H_*(M)$ we define
$$GW_{A,3}(a,b,c):=GW_{a,3}(PD(a),PD(b),PD(c)).$$
It counts the intersection number of the product class $a\times b\times c$ with the 
evaluation map $ev:\mathcal{M}_{0,3}^M(A;J)\to M^{\times 3}$, where 
$\mathcal{M}_{0,3}^M(A;J)$ is the moduli space of $J$-holomorphic spheres passing through 
oriented submanifolds $X_i\subset M$ in general position and dual to the classes $a,b$ 
and $c$.
This invariant is zero unless the sum of the degrees $PD(a)+PD(b)+PD(c)$ is equal to the 
dimension of the moduli space, which is $dim(M)+2c_1(A)$. 
\end{remark}

We start by computing the Chern classes. 
The adjunction formula tells us that for a homology class $C$ 
$$1+\frac{C\cdot C-c_1(C)}{2}=g.,$$
where $g$ is the genus of $C$.
For $C=\Sigma_2$ this yields
$1+\frac{2-c_1(\Sigma_2)}{2}=0$ and hence
$$c_1(\Sigma_2)=4.$$
Similarly for $C=F$ we get
$1+\frac{0-c_1(F)}{2}=0$ and hence
$$c_1(F)=2.$$
A curve in the class $s\Sigma_2+rF$ has therefor Chern class $s4+2r$, which is two if and 
only if $2s+r=0$. Using symplectic surgery one can show that a $J$-holomorphic curve in 
the class $\Sigma_2-F$ exists.
Positivity of intersection implies that there cannot exist holomorphic curves in the 
class $s\Sigma_2-rF$ for $(s,r)\neq (0,1) \text{ or } (1,-1)$. \begin{bf}How? 
symplectic surgery to get the curve $\Sigma_2-F$? positivity of intersection?\end{bf}

For the three point Gromov Witten 
invariants $GW_{A,3}(a,b,c)$ we have following possibilities for the degrees of the 
classes $a,b,c$ and for the homology classes $A$:
\begin{center}
  \begin{tabular}{ c || c | c }
    $c_1(A)$ & $\deg(a)+\deg(b)+\deg(c)$ & $A$ \\ \hline
    $0$ & $4+4+0$ or $2+2+4$ & $\text{constant curves}$  \\ 
    $2$ & $2+2+0$ or $4+0+0$ & $F$,$\Sigma_2-F$.   \\ 
    $4$ & $0+0+0$ & $\Sigma_2$. \\
  \end{tabular}
\end{center}
The case $c_1(A)=0$ is just the classical intersection product.
Consider the case $c_1(a)=2$. Since $[F]\cdot [F]=0$ we have
$$GW_{F}(F,F,p)=0 \text{ and } GW_F(F,\Sigma_2,p)=0.$$
For a generic point $p\in \mathbb{P}(\mathcal{O}(2)\oplus 
\mathcal{O})$ there exists exactly one fiber through $p$. Thus
$$GW_F(\Sigma_2,\Sigma_2,p)=2.$$
Moreover $[\Sigma_2\-F]\cdot [F]=1$ and $[\Sigma_2\-F]\cdot [\Sigma_2]=1$, hence we also 
have
$$GW_{\Sigma_2-F}(F,F,p)=1 , GW_{\Sigma_2-F}(F,\Sigma_2,p)=1 \text{ and } 
GW_{\Sigma_2-F}(\Sigma_2,\Sigma_2,p)=1.$$
As $U$ is the unit and $[F]\cdot [F]=0$ as well as $[\Sigma_2-F]\cdot[\Sigma_2-F]=0$ we 
conclude that $[Z_2]-[F]$ cannot pass trough two generic points and
$$GW_F(U,p,p)=GW_{\Sigma_2-F}(U,p,p)=0.$$
In the case $c_1(A)=4$ we easily see $GW_{\Sigma_2}(p,p,p)=0$.

To deduce the quantum product on $QH_*(F_0)$ notice that after collapsing 
$\Sigma_2\subset \mathbb{P}(\mathcal{O}(2)\oplus 
\mathcal{O})$ we get 
$$0=[\Sigma_{-2}]=[\Sigma_2-2F]$$ and hence
$$[\Sigma_2-F]=[F] \text{ and } [\Sigma_2]=2[F].$$
Hence there is only one three point Gromov Witten invariant $GW_{A,3}(a,b,c)$ with 
$c_1(A)=2$ and it is given by 
$$GW_{F}(F,F,p)=\frac{1}{4}GW_F(\Sigma_2,\Sigma_2,p)+GW_{\Sigma_2-f}(F,F,p)+\frac{1}{2} 
GW_{\Sigma_2-F}(F,F,p)+\frac{1}{4}GW_{\Sigma_2-F}(\Sigma_2,\Sigma_2,p)=2.$$
Hence $$[F]*[F]=2[U]q^2 \text{ and } p*[F]=4[F]q^2$$
and 
$$QH_*(F_0)=\frac{\mathbb{Z}[U]\oplus \mathbb{Z}[F]\oplus \mathbb{Z}p}{\langle 
[F]*[F]=2[U]q^2 , p*[F]=4[F]q^2, U \text{ the unit }\rangle} .$$
\end{example}


